Random Walk Guided Hyperbolic Graph Distillation

Graph distillation (GD) is an effective approach to extract useful information from large-scale network structures. However, existing methods, which operate in Euclidean space to generate condensed graphs, struggle to capture the inherent tree-like geometry of real-world networks, resulting in distilled graphs with limited task-specific information for downstream tasks. Furthermore, these methods often fail to extract dynamic properties from graphs, which are crucial for understanding information flow and facilitating graph continual learning. This paper presents the Hyperbolic Graph Distillation with Random Walks Optimization (HyDRO), a novel graph distillation approach that leverages hyperbolic embeddings to capture complex geometric patterns and optimize the spectral gap in hyperbolic space. Experiments show that HyDRO demonstrates strong task generalization, consistently outperforming state-of-the-art methods in both node classification and link prediction tasks. HyDRO also effectively preserves graph random walk properties, producing condensed graphs that achieve enhanced performance in continual graph learning. Additionally, HyDRO achieves competitive results on mainstream graph distillation benchmarks, while maintaining a strong balance between privacy and utility, and exhibiting robust resistance to noises.

==> tables/NAS2.tex <==
% \begin{table}
% % \vspace{8em}
% \centering
% \caption{NAS evaluation. The best results are in \textcolor{blue}{blue}. The runner-ups are {\ul underlined}. The worst results are colored \textcolor{red}{red}.}
% \resizebox{\linewidth}{!}{%
% \setlength{\tabcolsep}{2pt} % added by Wei to reduce the margin between columns
% \begin{tabular}{@{}lcccc|ccccccccccc@{}}
% \toprule
% \textbf{Metrics} & \textbf{Averaging} & \textbf{Random} & \textbf{Herding} & \textbf{K-Center}  & \textbf{GCond} & \textbf{SGDD}  & \textbf{DosCond}   & \textbf{MSGC} & \textbf{GCDM} & \textbf{GCSNTK} & \textbf{MSGC} &  \textbf{SFGC} & \textbf{GEOM} & \textbf{GDEM} & \textbf{HyDRO} \\ \midrule

% % Citeseer 0.25%
% Top 1 (\%)                     & 78.99           & 71.00             & {\color[HTML]{FF0000} 70.82}           & \textbf{66.79} & 81.8         & 75.66          & 81.91                       & {\ul 82.40}   & 82.30            & 81.85            & 82.10            & 81.92    & 81.92 & 81.92 & 81.60     

% \\
% Acc. Corr.                     & 0.34            & 0.22              & 0.19            & \textbf{0.13}  & 0.78          & 0.60           & {\color[HTML]{FF0000} -0.25} & {\ul 0.71}    & 0.68             & 0.62             & 0.70             & 0.67   & 0.34 & 0.67 & 0.64           \\
% Rank Corr.                     & 0.54            & 0.52              & 0.49            & 0.30           & {\ul 0.58}    & 0.13           & {\color[HTML]{FF0000} -0.17} & \textbf{0.78} & 0.75             & 0.70             & 0.73             & 0.72    & 0.67 & 0.67 & 0.48         \\ 


% % Pubmed 0.5%


% \midrule
% Top 1 (\%)                     & 70.00           & 47.92             & {\color[HTML]{FF0000} 60.22}           & \textbf{58.35} & 71.76         & 73.21          & 65.85                       & {\ul 82.40}   & 82.30            & 81.85            & 82.10            & 81.92    & 81.92 & 81.92 & 73.40     

% \\
% Acc. Corr.                     & 0.18            & 0.03              & 0.17            & \textbf{-0.36}  & 0.06          & 0.78           & {\color[HTML]{FF0000} 0.14} & {\ul 0.71}    & 0.68             & 0.62             & 0.70             & 0.67   & 0.34 & 0.67 & 0.77
% \\
% Rank Corr.                     & 0.50            & 0.47              & 0.55            & 0.14           & {\ul 0.45}    & 0.76           & {\color[HTML]{FF0000} 0.20} & \textbf{0.26} & 0.75             & 0.70             & 0.73             & 0.72    & 0.67 & 0.67 & 0.73         \\ 


% % Flickr 0.005%
% \midrule
% Top 1 (\%)                     & 81.88           & 81.74             & {\color[HTML]{FF0000} 81.49}           & \textbf{82.42} & 82.19         & 81.82          & 81.91                       & {\ul 82.40}   & 82.30            & 81.85            & 82.10            & 81.92    & 81.92 & 81.92 & 73.40     \\
% Acc. Corr.                     & 0.56            & 0.47              & 0.40            & \textbf{0.72}  & 0.65          & 0.70           & {\color[HTML]{FF0000} 0.14} & {\ul 0.71}    & 0.68             & 0.62             & 0.70             & 0.67   & 0.34 & 0.67 & 0.76           \\
% Rank Corr.                     & 0.64            & 0.60              & 0.57            & 0.71           & {\ul 0.74}    & 0.66           & {\color[HTML]{FF0000} 0.20} & \textbf{0.78} & 0.75             & 0.70             & 0.73             & 0.72    & 0.67 & 0.67 & 0.73         \\ 






% \bottomrule
% \end{tabular}%
% }
% \label{tab:NAS}
% % \vspace{-0.5em}
% \end{table}



\begin{table*}
\centering
\caption{NAS evaluation. The best results are in \textcolor{blue}{blue}. The runner-ups are {\ul underlined}. The worst results are colored \textcolor{red}{red}.}
\resizebox{\linewidth}{!}{%
\setlength{\tabcolsep}{2pt} % added by Wei to reduce the margin between columns
\begin{Huge}
\begin{tabular}{@{}l|lcccc|ccccccccccc@{}}
\toprule
\textbf{Dataset} & \textbf{Metrics} & \textbf{Averaging} & \textbf{Random} & \textbf{Herding} & \textbf{K-Center} & \textbf{GCond} & \textbf{SGDD} & \textbf{DosCond} & \textbf{MSGC} & \textbf{GCSNTK}  & \textbf{SFGC} & \textbf{GEOM} &  \textbf{HyDRO} \\ 
% \midrule

% \multirow{3}{*}{\centering Citeseer(0.9\%)} 
% & Top 1 (\%)                     & 70.00           & 47.92             & 60.22           & 58.35 & 71.76         & \textbf{73.03}                                & {\ul 65.84}   & 71.38            & 68.78                          & 42.51 & 70.75 & \textcolor{blue}{\textbf{73.4}} \\ 
% & Acc. Corr.                           & 18.21            & 3.29 & 17.09          & -36.31           &  62.39 & {\ul 22.94}    & 5.61             & 82.45             & -18.99             & 26.85   & \textbf{58.80}& \textcolor{blue}{\textbf{76.80}} \\ 
% & Rank Corr.                           & 49.71              & 47.18                      & {\ul 54.69}    & 14.25           & 44.69 & 55.33 & 26.27             & \textcolor{blue}{\textbf{79.69 }}            & -13.27             & 71.03    & 60.67 & \textbf{72.87} \\ 
\midrule

% Pubmed 0.5%
\multirow{3}{*}{\centering Pubmed(0.02\%)}
& Top 1 (\%)                               & 76.56             & 70.53           & 75.48 & 73.31         & 78.53                               & {\ul 78.34}   & 76.14            & 77.79            & 77.29            & 77.92    & \textcolor{blue}{\textbf{79.34}}  & \textbf{78.92} \\ 
& Acc. Corr.                              & 14.84            & 32.09  & 44.95          & 48.28           & \textbf{ 63.50} & \textcolor{blue}{\textbf{ 64.96}}    & 14.99             & 50.93             & 48.51             & 55.43    & 41.68 & 59.60 \\ 
& Rank Corr.                        & 20.65              & 51.17                       & {\ul 60.06}    & 60.58           & \textcolor{blue}{\textbf{ 82.88}} & 76.92 & 7.22            & 52.05             & 33.63             & 66.12    & 54.53 & \textbf{77.75} \\ 
% \midrule

% % Flickr 0.005%
% \multirow{3}{*}{\centering Flickr(0.005\%)}
% & Top 1 (\%)                    & 44.77             & 43.86         & 41.28 & 43.09               & \textbf{46.84}                      & {\ul 44.79}   & 46.72            & 46.76            & 46.01            & 44.24    & 46.35 & \textcolor{blue}{\textbf{46.90}} \\ 
% & Acc. Corr.                        & 72.40              & \textcolor{blue}{\textbf{87.94}}            & \textbf{87.56}           & 89.38          & 75.43 & {\ul 77.96}    & 84.07             & 75.69             & 70.31             & 86.68   & 85.59 & 80.80 \\ 
% & Rank Corr.                             & 73.08              & 72.09                    &\textbf{ 76.70}    & 74.19           & 70.61 & 66.24 & 76.43             & 73.14            & 69.33             & 73.79   & 71.18 & \textcolor{blue}{\textbf{80.11}} \\ 

\midrule

% DBLP 0.001%
\multirow{3}{*}{\centering DBLP(0.001\%)}
& Top 1 (\%)                                & \textcolor{blue}{\textbf{ 82.87}}           & 54.28 & 62.96         & 60.76         & 81.72                       & {\ul 80.79}   & \textbf{82.41}            & 84.25            & 79.65            & 63.68    & 71.58 & 82.10 \\ 
& Acc. Corr.                                  & \textbf{65.13 }           & 21.32  & 39.40          & 38.42          & 55.26 & {\ul 52.39}    & 51.67             & \textcolor{blue}{\textbf{73.63}}             & 43.11             & 52.07    & 50.04 & 63.54 \\ 
& Rank Corr.                     & 62.11              & 20.79                      & {\ul 37.93}    & 36.38           & 57.81 & 52.12 & 56.13             & 77.60             & 47.62             & \textbf{65.97}   & 63.25 & \textcolor{blue}{\textbf{68.62}} \\ 

\bottomrule
\end{tabular}%
\end{Huge}
}
\label{tab:NAS}
\end{table*}



==> tables/cgl.tex <==
\begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{figs/cgl.pdf}
    \caption{GC methods on baseline datasets under the continual graph learning setting.}
    \label{fig:cgl-supp}
\end{figure*}

==> tables/transfer.tex <==
\begin{table*}[h]
\centering
\caption{Experimental results for the {\bf cross-architecture setting} are presented, including mean accuracy and standard deviation. The best results are highlighted in \textcolor{blue}{\textbf{bold}}, while the second-best values are marked in \textbf{\textit{bold italic}}
}
\label{tab:cross_table_1}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tiny}
\begin{tabular}{cccccccccccc}
\cline{1-11}
                          &         & \multicolumn{7}{c}{Architectures}                & \multicolumn{2}{c}{Statistics}                                                                                        &  \\ \cline{3-11}
\multirow{-2}{*}{Datasets} & \multirow{-2}{*}{Methods} & SGC  & GCN & Cheby & SAGE & APPNP& GAT & SGFormer & \textbf{Average}  \\ \cline{1-11}
                    
                          & GCond     & 73.3 & 73.2 & 71.4  & 70.1  & 72.9 & 70.9 & 69.3 & \textbf{71.6 $\pm$ 1.6}          \\ 
                      
                          & SGDD     & 70.47 & 70.18 & 70.44  & 69.85  & 70.72 & 70.64 & 68.50 & \textbf{70.1 $\pm$ 0.8}          \\ 
                          & DosCond     & 64.49 & 68.28 & 51.75  & 60.30  & 50.52 & 47.12 & 38.30 & \textbf{54.4 $\pm$ 10.5}          \\ 
                         
                      
                        
        
                          & GCSNTK   & 62.31 & 62.05 & 60.97  & 65.73  & 61.65 & 65.73 & 53.24 & \textbf{61.7 $\pm$ 4.1}           \\ 
                          & MSGC   & 70.3 & 70.2 & 70.5  & 69.7  & 70.7 & 71.4 & 69.5 & \textbf{70.3 $\pm$ 0.6}           \\ 
                          % & SFGC   & 44.5 & 44.1 & 48.4  & 48.6  & 44.8 & 48.8 & 41.0 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & GEOM   & 65.9 & 65.0 & 65.7  & 62.9  & 65.5 & 67.5 & 60.9 & \textbf{64.8 $\pm$ 2.1}           \\ 
                        
\multirow{-10}{*}{Citeseer(0.5\%)}  & HyDRO    & 72.77 & 72.77 & 72.40  & 72.14  & 72.94 & 69.60 & 69.97 & \textbf{71.8 $\pm$ 1.4}  \\ 

\midrule
& GCond     & 84.3 & 85.1 & 78.7  & 79.1  & 83.4 & 80.0 & 80.5 & \textbf{81.6 $\pm$ 2.6}          \\ 
                      
                          & SGDD     & 81.26 & 80.08 & 80.80  & 81.82  & 81.10 & 79.39 & 79.68 & \textbf{80.6 $\pm$ 0.9}          \\ 
                          & DosCond     & 81.72 & 82.96 & 81.39  & 81.56  & 81.27 & 80.37 & 73.95 & \textbf{80.5 $\pm$ 2.9}          \\ 
                         
                         
                        
        
                          & GCSNTK   & 77.81 & 77.95 & 80.04  & 80.12  & 80.51 & 79.82 & \textcolor{red}{71.36} & \textbf{79.4 $\pm$ 1.2}           \\ 
                          & MSGC   & 84.9 & 84.8 & 84.0  & 83.8  & 84.9 & 74.2 & 70.7 & \textbf{81.0 $\pm$ 5.9}           \\ 
                          % & SFGC   & 71.9 & 71.85 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & GEOM   & 82.7 & 83.4 & 81.7  & 81.9  & 83.1 & 81.9 & 81.6 & \textbf{82.3 $\pm$ 0.7}           \\ 
                          & GDEM   & 82.7 & 83.4 & 81.7  & 81.9  & 83.1 & 81.9 & 81.6 & \textbf{82.3 $\pm$ 0.7}           \\ 
                        
\multirow{-10}{*}{DBLP(0.01\%)}  & HyDRO    & 82.99 & 83.04 & 81.14  & 81.42  & 82.79 & 80.72 & 81.65 & \textbf{82.0 $\pm$ 0.9}  \\ 

% \midrule
% & GCond     & 78.0 & 76.7 & 77.3  & 76.5  & 77.8 & 76.0 & 71.5 & \textbf{76.2 $\pm$ 2.2}          \\ 
                      
%                           & SGDD     & 78.51 & 76.42 & 76.70  & 76.25  & 78.60 & 75.78 & 70.60 & \textbf{76.1 $\pm$ 2.6}          \\ 
%                           & DosCond     & 75.01 & 77.67 & 74.87  & 71.56  & 76.31 & 68.56 & 69.34 & \textbf{73.3 $\pm$ 3.5}          \\ 
                        
%                           & GCSNTK   & 77.13 & 75.80 & 74.34  & 76.29  & 76.21 & 76.82 & \textcolor{red}{71.36} & \textbf{76.1 $\pm$ 1.0}            \\ 
%                           & MSGC   & 78.3 & 78.1 & 77.0  & 76.9  & 78.8 & 76.3 & 74.2 & \textbf{77.1 $\pm$ 1.5}           \\ 
%                           % & SFGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
%                           & GEOM   & 78.6 & 78.4 & 78.2  & 77.3  & 78.4 & 78.04 & 77.98 & \textbf{78.1 $\pm$ 0.4}           \\ 
                        
% \multirow{-10}{*}{Pubmed(0.5\%)}  & HyDRO    & 78.53 & 78.24 & 78.01  & 77.35  & 78.6 & 77.97 & 76.97 & \textbf{78.0 $\pm$ 0.6}  \\ 



\cline{1-11}

\end{tabular}%
\end{tiny}
}
\end{table*}


% citeseer 0.5
% dblp0.01
% pubmed 0.5

==> tables/transfer2.tex <==
\begin{table*}[h]
\centering
\caption{Results of cross-architecture setting, we test condensed graphs in APPNP, Cheby, GCN, GraphSAGE, and SGC. Avg. and Std.: the average performance and the standard deviation of the results. We mark the best performance by \textbf{bold}.}
\label{tab:cross_table_1}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{Huge}
\begin{tabular}{cccccccccccc}
\cline{1-11}
                          &         & \multicolumn{7}{c}{Architectures}                & \multicolumn{2}{c}{Statistics}                                                                                        &  \\ \cline{3-11}
\multirow{-2}{*}{Datasets} & \multirow{-2}{*}{Methods} & SGC~\cite{wu2019simplifying}  & GCN~\cite{kipf2016semi}  & Cheby~\cite{defferrard2016convolutional} & SAGE~\cite{hamilton2017inductive} & APPNP~\cite{klicpera2018predict-appnp}  & GAT~\cite{gat} & SGFormer~\cite{MLP}  & \textbf{Average}  \\ \cline{1-11}
                    
                          & GCond     & 50.3 & 54.8 & 81.2  & 77.5  & 89.5 & 89.7 & 90.5 & \textbf{76.2 $\pm$ 16.9}          \\ 
                      
                          & SGDD     & 70.47 & 70.18 & 70.44  & 69.85  & 70.72 & 70.64 & 68.50 & \textbf{76.2 $\pm$ 16.9}          \\ 
                          & DosCond     & 64.49 & 68.28 & 51.75  & 60.30  & 50.52 & 47.12 & 38.30 & \textbf{76.2 $\pm$ 16.9}          \\ 
                         
                      
                        
        
                          & GCSNTK   & 62.31 & 62.05 & 60.97  & 65.73  & 61.65 & 65.73 & 53.24 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & MSGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & SFGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & GEOM   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                        
\multirow{-10}{*}{Citeseer(0.5\%)~\cite{hamilton2017inductive}}  & HyDRO    & 72.77 & 72.77 & 72.40  & 72.14  & 72.94 & 69.60 & 69.97 & \textbf{80.9 $\pm$ 12.6}  \\ 

\midrule
& GCond     & 50.3 & 54.8 & 81.2  & 77.5  & 89.5 & 89.7 & 90.5 & \textbf{76.2 $\pm$ 16.9}          \\ 
                      
                          & SGDD     & 81.26 & 80.08 & 80.80  & 81.82  & 81.10 & 79.39 & 79.68 & \textbf{76.2 $\pm$ 16.9}          \\ 
                          & DosCond     & 81.72 & 82.96 & 81.39  & 81.56  & 81.27 & 80.37 & 73.95 & \textbf{76.2 $\pm$ 16.9}          \\ 
                         
                         
                        
        
                          & GCSNTK   & 77.81 & 77.95 & 80.04  & 80.12  & 80.51 & 79.82 & \textcolor{red}{71.36} & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & MSGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & SFGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & GEOM   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                        
\multirow{-10}{*}{DBLP(0.01\%)~\cite{hamilton2017inductive}}  & HyDRO    & 82.99 & 83.04 & 81.14  & 81.42  & 82.79 & 80.72 & 81.65 & \textbf{80.9 $\pm$ 12.6}  \\ 

\midrule
& GCond     & 50.3 & 54.8 & 81.2  & 77.5  & 89.5 & 89.7 & 90.5 & \textbf{76.2 $\pm$ 16.9}          \\ 
                      
                          & SGDD     & 78.51 & 76.42 & 76.70  & 76.25  & 78.60 & 75.78 & 70.60 & \textbf{76.2 $\pm$ 16.9}          \\ 
                          & DosCond     & 75.01 & 77.67 & 74.87  & 71.56  & 76.31 & 68.56 & 69.34 & \textbf{76.2 $\pm$ 16.9}          \\ 
                        
                          & GCSNTK   & 77.13 & 75.80 & 74.34  & 76.29  & 76.21 & 76.82 & \textcolor{red}{71.36} & \textbf{76.3 $\pm$ 18.5}            \\ 
                          & MSGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & SFGC   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                          & GEOM   & 42.5 & 60.2 & 87.8  & 75.5  & 89.4 & 89.1 & 89.6 & \textbf{76.3 $\pm$ 18.5}           \\ 
                        
\multirow{-10}{*}{Pubmed(0.5\%)~\cite{hamilton2017inductive}}  & HyDRO    & 78.53 & 78.24 & 78.01  & 77.35  & 89.4 & 78.60 & 76.97 & \textbf{80.9 $\pm$ 12.6}  \\ 



\cline{1-11}

\end{tabular}%
\end{Huge}
}
\end{table*}


% citeseer 0.5
% dblp0.01
% pubmed 0.5
